HVH: Learning a Hybrid Neural Volumetric Representation for Dynamic Hair Performance Capture

Capturing and rendering life-like hair is particularly challenging due to its fine geometric structure, the complex physical interaction and its non-trivial visual appearance.Yet, hair is a critical component for believable avatars. In this paper, we address the aforementioned problems: 1) we use a novel, volumetric hair representation that is com-posed of thousands of primitives. Each primitive can be rendered efficiently, yet realistically, by building on the latest advances in neural rendering. 2) To have a reliable control signal, we present a novel way of tracking hair on the strand level. To keep the computational effort manageable, we use guide hairs and classic techniques to expand those into a dense hood of hair. 3) To better enforce temporal consistency and generalization ability of our model, we further optimize the 3D scene flow of our representation with multi-view optical flow, using volumetric ray marching. Our method can not only create realistic renders of recorded multi-view sequences, but also create renderings for new hair configurations by providing new control signals. We compare our method with existing work on viewpoint synthesis and drivable animation and achieve state-of-the-art results. Please check out our project website at https://ziyanw1.github.io/hvh/.

==> conclusion.tex <==
\section{Conclusion}

In this paper, we present a hybrid neural volumetric representation for hair dynamic performance capture. Our representation leverages the efficiency of guide hair representation in hair simulation by attaching volumetric primitives to them as well as the high DoF of volumetric representation. The hybrid volumetric representation could be regressed from a global temporal latent code and per-strand hair features with hair structure awareness and it is optimized using multiview RGB images and optical flows. We show that our method could generate sharper and higher quality results on hair and our method achieves better generalization with temporal consistency.
